EAST: Early Action Prediction Sampling Strategy with Token Masking

Early action prediction seeks to anticipate an action before it fully unfolds, but limited visual evidence makes this task especially challenging. We introduce EAST, a simple and efficient framework that enables a model to reason about incomplete observations. In our empirical study, we identify key components when training early action prediction models. Our key contribution is a randomized training strategy that samples a time step separating observed and unobserved video frames, enabling a single model to generalize seamlessly across all test-time observation ratios. We further show that joint learning on both observed and future (oracle) representations significantly boosts performance, even allowing an encoder-only model to excel. To improve scalability, we propose a token masking procedure that cuts memory usage in half and accelerates training by 2x with negligible accuracy loss. Combined with a forecasting decoder, EAST sets a new state of the art on NTU60, SSv2, and UCF101, surpassing previous best work by 10.1, 7.7, and 3.9 percentage points, respectively.

==> tab/sub21_A.tex <==
\begin{table*}
  \centering
  \begin{tabular}{lrrrrrrrrr}
    \toprule
    Method & 0.1 & 0.2 & 0.3 & 0.4 & 0.5 & 0.6 & 0.7 & 0.8 & 0.9 \\
    \midrule
    MS-LSTM $\dagger$~\cite{sadegh17iccv} & 16.9 & 16.6 & 16.8 & - & 16.7 & - & 16.9 & - & 17.1 \\
    MSRNN $\dagger$~\cite{sadegh17iccv} & 20.1 & 20.5 & 21.1 & - & 22.5 & - & 24.0 & - & 27.1 \\
     mem-LSTM $\dagger$~\cite{kong18aaai}& 14.9 & 17.2 & 18.1 & - & 20.4 & - & 23.2 & - & 24.5 \\
    GGN~\cite{wu21aaai} & 21.2 & 21.5&23.3&-&27.7&-&30.2&-&30.6\\
    IGGN~\cite{wu21ijcv}& 22.6 & -&25.0& - &28.3&-&32.2&-&34.1\\
    TempPr\cite{Stergiou23CVPR} & 28.4 & 34.8 & 37.9 & - & 41.3 & - & 45.8&-&48.6\\
    % Ours w/o masking &  & &&&70.87?&&&&&\\
    % Ours w diff masking &  &&&&69.10&&&&&\\
    ASAP (ours) & \textbf{42.5}  & \textbf{46.3}&\textbf{50.7}&\textbf{57.7}&\textbf{64.0}&\textbf{70.7}&\textbf{74.3}&\textbf{79.1}&\textbf{81.3}\\
    % Ours w diff masking & 42.50  & 46.33&50.72&57.66&63.97&70.67&74.31&79.08
    % &81.3&\\
    \bottomrule
  \end{tabular}
  \caption{Results on SSsub21. $\dagger$ means that results are taken from~\cite{Stergiou23CVPR}}
  \label{tab:sub21_main}
\end{table*}

==> tab/ucf101_main_backup.tex <==
\begin{table*}
  \centering
  \small
  \setlength{\tabcolsep}{1mm}
  \begin{tabular}{lrrrrrrrrrrr}
    \toprule
    & \multicolumn{9}{c}{Observation ratio $\rho$} \\
    Method &encoder& 0.1 & 0.2 & 0.3 & 0.4 & 0.5 & 0.6 & 0.7 & 0.8 & 0.9 & avg\\
    \midrule
    % MSSC*~\cite{cao13cvpr}&ResNet-18& 34.1& 53.8& 58.3& 57.6& 62.6& 61.9& 63.5& 64.3& 62.7&57.6\\
    MSSC*&ResNet-18& 34.1& 53.8& 58.3& 57.6& 62.6& 61.9& 63.5& 64.3& 62.7&57.6\\
    % MTSSVM*~\cite{kong14eccv} &ResNet-18&40.1& 72.8& 80.0& 82.2& 82.4& 83.2& 83.4& 83.6& 83.7&76.8\\ 
    MTSSVM*&ResNet-18&40.1& 72.8& 80.0& 82.2& 82.4& 83.2& 83.4& 83.6& 83.7&76.8\\ 
    % DeepSCN~\cite{kong17cvpr}&ResNet-18& 45.0& 77.7& 83.0& 85.4& 85.8& 86.7& 87.1& 87.4& 87.5&80.6\\
    DeepSCN&ResNet-18& 45.0& 77.7& 83.0& 85.4& 85.8& 86.7& 87.1& 87.4& 87.5&80.6\\
    % DeepSCN~\cite{kong17cvpr} &45.0 &77.7& 83.0& 85.4& 85.8& 86.7& 87.1& 87.4 &87.5\\
    MSRNN&ResNet-18& 68.0& 87.2& 88.2& 88.8& 89.2& 89.7& 89.9& 90.3 &90.4&86.6\\
    % MSRNN~\cite{sadegh17iccv}&ResNet-18& 68.0& 87.2& 88.2& 88.8& 89.2& 89.7& 89.9& 90.3 &90.4&86.6\\
    % mem-LSTM~\cite{kong18aaai}&ResNet-18& 51.0& 81.0& 85.7& 85.8& 88.4& 88.6& 89.1& 89.4& 89.7&83.2\\
    mem-LSTM&ResNet-18& 51.0& 81.0& 85.7& 85.8& 88.4& 88.6& 89.1& 89.4& 89.7&83.2\\
    % AAPNET~\cite{kong18pami}&C3D& 59.9& 80.4& 86.8& 86.5& 86.9& 88.3& 88.3& 89.9& 90.9&84.2\\
    AAPNET&C3D& 59.9& 80.4& 86.8& 86.5& 86.9& 88.3& 88.3& 89.9& 90.9&84.2\\
    % RGN-KF~\cite{zhao19iccv} &Inception&83.3 &85.2& 87.8& 90.6& 91.5& 92.3& 92.0& 93.0 &92.9 &89.8 \\
    RGN-KF &Inception&83.3 &85.2& 87.8& 90.6& 91.5& 92.3& 92.0& 93.0 &92.9 &89.8 \\
    % DBDNet~\cite{pang19ijcai} &ResNeXt101& 82.7 &86.6& 88.4& 89.7& 90.6 &91.1 &91.7& 91.9& 92.0 &89.4\\
    DBDNet &ResNeXt101& 82.7 &86.6& 88.4& 89.7& 90.6 &91.1 &91.7& 91.9& 92.0 &89.4\\
    % AA-GAN~\cite{gammulle19iccv}&ResNet-50& - &84.2& - &- &85.6& -& - &- &-&-\\
    AA-GAN&ResNet-50& - &84.2& - &- &85.6& -& - &- &-&-\\
    % TS~\cite{Wang19CVPR} &Inception& 83.3 & 87.1 & 88.9 & 89.9& 90.9 & 91.0 & 91.3 & 91.2 & 91.3 &89.4\\
    TS &Inception& 83.3 & 87.1 & 88.9 & 89.9& 90.9 & 91.0 & 91.3 & 91.2 & 91.3 &89.4\\
    % GGNN~\cite{wu21aaai} &ResNet-50& 84.1 &88.5 &89.8 &- &90.9 &- &91.4 &- &91.8&-\\
    GGNN &ResNet-50& 84.1 &88.5 &89.8 &- &90.9 &- &91.4 &- &91.8&-\\
    % IGGN~\cite{wu21ijcv} &ResNeXt101& 80.2 & - & 89.8 & - & 92.9 & - & 94.1 & - & 94.4 &-\\
    IGGN &ResNeXt101& 80.2 & - & 89.8 & - & 92.9 & - & 94.1 & - & 94.4 &-\\
    % JVS + JCC + JFIP\cite{fernando21cvpr}(RGB+flow) & - & 91.7 & - & - & - & - & - & - & - \\
    % JVS~\cite{fernando21cvpr} &ResNet-50& - & 91.7 & - & - & - & - & - & - & -&- \\
    JVS &ResNet-50& - & 91.7 & - & - & - & - & - & - & -&- \\
    % ERA~\cite{foo22eccv} &ResNeXt101& 89.1 & - & 92.4 & - & 94.2 & - &95.5 & - & 95.7 &-\\
    ERA &ResNeXt101& 89.1 & - & 92.4 & - & 94.2 & - &95.5 & - & 95.7 &-\\
    % \rowcolor{gray!20}
    % \underline{TempPr~\cite{Stergiou23CVPR}}  &\underline{MoViNet}& \underline{88.6} & \underline{93.5} & \underline{94.9} & \underline{94.9} & \underline{95.4} & \underline{95.2} & \underline{95.3}&\underline{96.6}&\underline{96.2}&\underline{94.5}\\
    \underline{TempPr}  &\underline{MoViNet}& \underline{88.6} & \underline{93.5} & \underline{94.9} & \underline{94.9} & \underline{95.4} & \underline{95.2} & \underline{95.3}&\underline{96.6}&\underline{96.2}&\underline{94.5}\\
    % TempPr~\cite{Stergiou23CVPR} $\dagger$&MoViNet & 85.1 & - & 90.4 & -& 92.5 & -& 92.8&-&93.2&\\
    TempPr $\dagger$&MoViNet & 85.1 & - & 90.4 & -& 92.5 & -& 92.8&-&93.2&\\
    % Ours w/o masking &  & &&&&&&&&\\
    % \rowcolor{gray!20}
    % ASAP (ours) & \textbf{89.6} & 90.7&92.3&92.7&93.3&93.5&93.4&93.4&93.6&\\
    %\midrule
    %ASAP w MoViNet-A4 & 89.5 &92.6 &93.1&93.1&94.0&94.8&95.3&&94.8\\
    %ASAP w MoViNet-A4 & 89.5 &92.6 &93.1&93.1&94.0&94.8&95.3&&94.8\\
    % Ours w random masking &  & &&&&&&&&\\
    % \bottomrule
    \hline
    % \ours~(ViT - GPT2(4L)&88.7 &91.3 & 91.8 & 92.7 & 93.3 & 93.5 & 93.6 & 93.6 & 93.6\\
    % Ours (MoViNet - GPT2(4L))&90.8&92.7&93.7&94.4&95.3&95.3&95.5&95.5&95.5\\
    % Ours (MoViNet - GPT2(12L))&&&&&&&&&\\
    % Ours (MoViNet - ViT(4L))&91.1&92.6&93.3&94.5&95.2&95.6&95.9&95.9&96.0\\
    \ours~&VideoMAE&88.6&91.4&92.2&93.1&93.4&93.6&93.7&93.8&93.8&92.6\\
    \ours~&MoViNet&\textbf{91.3}&\textbf{93.2}&\textbf{93.8}&\textbf{94.7}&\textbf{95.5}&\textbf{96.1}&\textbf{96.4}&\textbf{96.5}&\textbf{96.5}&\textbf{94.9}\\
    
    
    % Ours (MoViNet - encoder only - present)&&&&&&&&&\\
    % Ours (MoViNet - encoder only - present+oracle)&88.7&90.7&91.8&92.6&93.8&94.4&94.3&94.4&94.5\\
    % Ours (ViT - encoder only - present+attn)&87.6&90.3&91.3&92.4&92.9&93.2&93.2&93.2&93.2\\
    
  \end{tabular}
  \caption{
    Comparison with the state-of-the-art results on UCF101 dataset.
    We show top-1 accuracies (\%) for early action prediction over different observation ratios.
    * denotes results on UCF101 that were not reported in the original paper, but are presented in~\cite{kong17cvpr}.
    Using original source code, we were unable to replicate the results reported in the~\cite{Stergiou23CVPR}. These results are underlined.
    % \colorbox{gray!20}{Gray} 
    $\dagger$ represents our corrected reproduction.
  }
  \label{tab:ucf101_main_backup}
\end{table*}

==> tab/wall_clock_A.tex <==
\begin{table}[H]
  \centering
  % \footnotesize
  % \small
  % \setlength{\tabcolsep}{3pt}
  \begin{tabular}{lr}
  % \centering
  % \begin{tabular}{l|lllllllll}
     \toprule
    
    &wall clock time per epoch \\
    \midrule
    TemPr &529 sec \\
    % \ours~$s_{o}$ &13.8 &    18.4 &   23.8 &  33.2 &  43.1 & 51.9 &   58.6 &  62.8 &  64.2\\
    % w rand m&23min&0.49&19.2&25.4&29.6&34.3&41.1&48.8&55.3&59.7&63.1&64.1\\
    \ours & 151 sec\\
    \bottomrule
  \end{tabular}
  \caption{
    Wall clock time for training on the UCF101 dataset comparing previous state-of-the-art Tempr and~\ours.
    }
  \label{tab:wall_clock_A}
\end{table}
